WorldGen: From Text to Traversable and Interactive 3D Worlds

We introduce WorldGen, a system that enables the automatic creation of large-scale, interactive 3D worlds directly from text prompts. Our approach transforms natural language descriptions into traversable, fully textured environments that can be immediately explored or edited within standard game engines. By combining LLM-driven scene layout reasoning, procedural generation, diffusion-based 3D generation, and object-aware scene decomposition, WorldGen bridges the gap between creative intent and functional virtual spaces, allowing creators to design coherent, navigable worlds without manual modeling or specialized 3D expertise. The system is fully modular and supports fine-grained control over layout, scale, and style, producing worlds that are geometrically consistent, visually rich, and efficient to render in real time. This work represents a step towards accessible, generative world-building at scale, advancing the frontier of 3D generative AI for applications in gaming, simulation, and immersive social environments.

==> figures/fig_navmesh_illustration.tex <==
\begin{wrapfigure}[10]{r}{0.35\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figures_draft/navmesh_fig3.pdf}
\caption{a NavMesh extracted (colored in pink) from a 3D scene layout.}%\
\label{fig:navmesh_illustration}
\end{wrapfigure}


==> figures/fig_teaser.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.99\linewidth]{assets/teasers/teaser_hq.jpg}% chktex 8
\caption{\dilin{to be replaced. this will be replaced with high quality 2d renders from Milton}We present WorldGen, a system for generating traversable, interactive 3D worlds from text prompts. \thu{Optional: can we use another scene where the scale issue is not too obvious? the red/pink cars are at various scales here}
}%
\label{fig:teaser}
\end{figure}

